Ask About the Right Moment: Training-Free Object Identity Reasoning for Video-Language Models

Many questions about a video concern one physical object. Where does the ball end up after the cups are shuffled? Which card is the queen? How often was the mug covered? Open video-language models (Video-LMs) recognise such objects in single frames but do not keep them apart over time. On shuffled shell games, open models from eight families stay near chance, and so do published tool agents. We separate semantic identity binding from temporal identity maintenance. Binding should happen at a moment when the evidence for the object is visible, and maintenance should be left to a tracker. Track, Then Bind implements this principle without training. A promptable video tracker follows every candidate object and draws it with a track number. A frozen vision-language model (VLM) answers one question about the identifying evidence, which binds the target to a track. The answer is then derived from a text description of the tracks. With Qwen3-VL-32B, the agent solves both VET-Bench tasks, where a fine-tuned trajectory model reaches 92% and 90%. On real cup games from the Perception Test, it raises accuracy from 35.5% to 52.3%. Without retuning, the same configuration also solves VET-Bench with Gemma 4 and GPT-5.5. Its track-derived visibility timelines add 8.8-17.9 points on TOC-Bench for open models. GPT-6.1 already answers 92.5% of the real cup games directly but 71.0% through our pipeline, while our timelines still raise its TOC-Bench accuracy from 52.5% to 57.7%. The benefit of external tracking thus depends on the underlying model and the task.

==> figs/ex3/toc/timeline_fig2.tex <==
% Visibility timeline of TOC 8b0c33d38075 ('eggs'), data from benchmarks/examples/toc_timeline_export.py, drawn by make_timeline_tikz.py.
% Path commands for figs/pipeline.tex: plot area (0.18,0)-(4.02,-0.66), quantity above, ticks left and below.
\definecolor{tlFull}{HTML}{3A9A4A}\definecolor{tlPart}{HTML}{9FD29A}\definecolor{tlNone}{HTML}{BBBBBB}
\fill[tlFull] (0.180,-0.660) rectangle (0.376,0);
\fill[tlPart] (0.376,-0.660) rectangle (0.474,0);
\fill[tlNone] (0.474,-0.660) rectangle (0.645,0);
\fill[tlPart] (0.645,-0.660) rectangle (0.669,0);
\fill[tlFull] (0.669,-0.660) rectangle (1.501,0);
\fill[tlPart] (1.501,-0.660) rectangle (1.525,0);
\fill[tlFull] (1.525,-0.660) rectangle (1.550,0);
\fill[tlPart] (1.550,-0.660) rectangle (1.599,0);
\fill[tlFull] (1.599,-0.660) rectangle (3.409,0);
\fill[tlPart] (3.409,-0.660) rectangle (3.433,0);
\fill[tlNone] (3.433,-0.660) rectangle (3.678,0);
\fill[tlPart] (3.678,-0.660) rectangle (3.702,0);
\fill[tlFull] (3.702,-0.660) rectangle (3.751,0);
\fill[tlPart] (3.751,-0.660) rectangle (3.898,0);
\fill[tlFull] (3.898,-0.660) rectangle (4.020,0);
\draw[black,line width=0.5pt,line join=round] plot coordinates {(0.192,-0.162) (0.217,-0.162) (0.241,-0.162) (0.266,-0.162) (0.290,-0.155) (0.315,-0.157) (0.339,-0.155) (0.363,-0.217) (0.388,-0.374) (0.412,-0.452) (0.437,-0.520) (0.461,-0.584) (0.486,-0.601) (0.510,-0.609) (0.535,-0.612) (0.559,-0.611) (0.584,-0.621) (0.608,-0.623) (0.632,-0.618) (0.657,-0.552) (0.681,-0.160) (0.706,-0.168) (0.730,-0.161) (0.755,-0.158) (0.779,-0.162) (0.804,-0.163) (0.828,-0.163) (0.853,-0.163) (0.877,-0.163) (0.902,-0.170) (0.926,-0.170) (0.950,-0.171) (0.975,-0.171) (0.999,-0.171) (1.024,-0.163) (1.048,-0.163) (1.073,-0.162) (1.097,-0.162) (1.122,-0.162) (1.146,-0.162) (1.171,-0.171) (1.195,-0.171) (1.219,-0.170) (1.244,-0.162) (1.268,-0.163) (1.293,-0.158) (1.317,-0.166) (1.342,-0.185) (1.366,-0.313) (1.391,-0.334) (1.415,-0.282) (1.440,-0.286) (1.464,-0.318) (1.489,-0.350) (1.513,-0.363) (1.537,-0.351) (1.562,-0.366) (1.586,-0.356) (1.611,-0.162) (1.635,-0.162) (1.660,-0.163) (1.684,-0.162) (1.709,-0.160) (1.733,-0.160) (1.758,-0.160) (1.782,-0.160) (1.806,-0.166) (1.831,-0.159) (1.855,-0.163) (1.880,-0.170) (1.904,-0.163) (1.929,-0.163) (1.953,-0.171) (1.978,-0.171) (2.002,-0.171) (2.027,-0.163) (2.051,-0.163) (2.076,-0.171) (2.100,-0.163) (2.124,-0.163) (2.149,-0.163) (2.173,-0.163) (2.198,-0.163) (2.222,-0.159) (2.247,-0.156) (2.271,-0.156) (2.296,-0.290) (2.320,-0.338) (2.345,-0.347) (2.369,-0.309) (2.394,-0.291) (2.418,-0.261) (2.442,-0.233) (2.467,-0.223) (2.491,-0.226) (2.516,-0.236) (2.540,-0.242) (2.565,-0.241) (2.589,-0.242) (2.614,-0.238) (2.638,-0.159) (2.663,-0.158) (2.687,-0.167) (2.711,-0.163) (2.736,-0.170) (2.760,-0.169) (2.785,-0.170) (2.809,-0.169) (2.834,-0.164) (2.858,-0.163) (2.883,-0.159) (2.907,-0.161) (2.932,-0.161) (2.956,-0.160) (2.981,-0.157) (3.005,-0.152) (3.029,-0.152) (3.054,-0.150) (3.078,-0.148) (3.103,-0.148) (3.127,-0.148) (3.152,-0.148) (3.176,-0.148) (3.201,-0.148) (3.225,-0.148) (3.250,-0.148) (3.274,-0.148) (3.298,-0.148) (3.323,-0.148) (3.347,-0.148) (3.372,-0.149) (3.396,-0.148) (3.421,-0.370) (3.445,-0.602) (3.470,-0.614) (3.494,-0.615) (3.519,-0.620) (3.543,-0.625) (3.568,-0.625) (3.592,-0.619) (3.616,-0.613) (3.641,-0.609) (3.665,-0.603) (3.690,-0.555) (3.714,-0.265) (3.739,-0.178) (3.763,-0.464) (3.788,-0.593) (3.812,-0.497) (3.837,-0.469) (3.861,-0.483) (3.885,-0.444) (3.910,-0.234) (3.934,-0.235) (3.959,-0.222) (3.983,-0.220) (4.008,-0.228)};
\draw[black,line width=0.35pt,dash pattern=on 1.6pt off 1.1pt] (0.180,-0.355) -- (4.020,-0.355);
\draw[black,line width=0.45pt,dash pattern=on 0.4pt off 0.9pt] (0.180,-0.599) -- (4.020,-0.599);
\draw[black,line width=0.35pt] (0.180,-0.660) rectangle (4.020,0);
\draw[black,line width=0.35pt] (0.180,-0.660) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,small] at (0.180,-0.710) {0};
\draw[black,line width=0.35pt] (0.914,-0.660) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,small] at (0.914,-0.710) {5};
\draw[black,line width=0.35pt] (1.648,-0.660) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,small] at (1.648,-0.710) {10};
\draw[black,line width=0.35pt] (2.381,-0.660) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,small] at (2.381,-0.710) {15};
\draw[black,line width=0.35pt] (3.115,-0.660) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,small] at (3.115,-0.710) {20};
\draw[black,line width=0.35pt] (3.849,-0.660) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,small] at (3.849,-0.710) {25\,s};
\draw[black,line width=0.35pt] (0.180,-0.660) -- ++(-0.05,0);
\node[anchor=east,inner sep=0.8pt,small] at (0.130,-0.660) {0};
\draw[black,line width=0.35pt] (0.180,-0.152) -- ++(-0.05,0);
\node[anchor=east,inner sep=0.8pt,small] at (0.130,-0.152) {1};
\node[anchor=south west,inner sep=0.8pt,small] at (0.150,0) {area / p90};


==> figs/ex3/toc/timeline_fig9.tex <==
% Visibility timeline of TOC 8b0c33d38075 ('eggs'), data from benchmarks/examples/toc_timeline_export.py, drawn by make_timeline_tikz.py.
% Complete picture for the step-5 card of figs/walk_toc.tex (5.4 cm wide).
\begin{tikzpicture}[x=1cm,y=1cm,every node/.style={}]
\definecolor{tlFull}{HTML}{3A9A4A}\definecolor{tlPart}{HTML}{9FD29A}\definecolor{tlNone}{HTML}{BBBBBB}
\fill[tlFull] (0.620,-1.150) rectangle (0.864,0);
\fill[tlPart] (0.864,-1.150) rectangle (0.985,0);
\fill[tlNone] (0.985,-1.150) rectangle (1.198,0);
\fill[tlPart] (1.198,-1.150) rectangle (1.229,0);
\fill[tlFull] (1.229,-1.150) rectangle (2.264,0);
\fill[tlPart] (2.264,-1.150) rectangle (2.295,0);
\fill[tlFull] (2.295,-1.150) rectangle (2.325,0);
\fill[tlPart] (2.325,-1.150) rectangle (2.386,0);
\fill[tlFull] (2.386,-1.150) rectangle (4.639,0);
\fill[tlPart] (4.639,-1.150) rectangle (4.669,0);
\fill[tlNone] (4.669,-1.150) rectangle (4.974,0);
\fill[tlPart] (4.974,-1.150) rectangle (5.004,0);
\fill[tlFull] (5.004,-1.150) rectangle (5.065,0);
\fill[tlPart] (5.065,-1.150) rectangle (5.248,0);
\fill[tlFull] (5.248,-1.150) rectangle (5.400,0);
\draw[black,line width=0.5pt,line join=round] plot coordinates {(0.635,-0.283) (0.666,-0.282) (0.696,-0.282) (0.727,-0.282) (0.757,-0.269) (0.787,-0.273) (0.818,-0.271) (0.848,-0.377) (0.879,-0.652) (0.909,-0.788) (0.940,-0.906) (0.970,-1.017) (1.001,-1.047) (1.031,-1.061) (1.061,-1.066) (1.092,-1.065) (1.122,-1.082) (1.153,-1.086) (1.183,-1.077) (1.214,-0.961) (1.244,-0.278) (1.275,-0.292) (1.305,-0.281) (1.335,-0.275) (1.366,-0.283) (1.396,-0.283) (1.427,-0.284) (1.457,-0.285) (1.488,-0.283) (1.518,-0.297) (1.549,-0.297) (1.579,-0.297) (1.609,-0.297) (1.640,-0.298) (1.670,-0.284) (1.701,-0.283) (1.731,-0.283) (1.762,-0.283) (1.792,-0.283) (1.823,-0.283) (1.853,-0.298) (1.884,-0.297) (1.914,-0.297) (1.944,-0.282) (1.975,-0.283) (2.005,-0.276) (2.036,-0.289) (2.066,-0.322) (2.097,-0.546) (2.127,-0.582) (2.158,-0.491) (2.188,-0.499) (2.218,-0.554) (2.249,-0.610) (2.279,-0.632) (2.310,-0.612) (2.340,-0.637) (2.371,-0.621) (2.401,-0.282) (2.432,-0.283) (2.462,-0.284) (2.492,-0.282) (2.523,-0.279) (2.553,-0.278) (2.584,-0.278) (2.614,-0.279) (2.645,-0.289) (2.675,-0.277) (2.706,-0.285) (2.736,-0.297) (2.766,-0.283) (2.797,-0.284) (2.827,-0.298) (2.858,-0.298) (2.888,-0.298) (2.919,-0.284) (2.949,-0.284) (2.980,-0.298) (3.010,-0.284) (3.040,-0.285) (3.071,-0.284) (3.101,-0.283) (3.132,-0.284) (3.162,-0.277) (3.193,-0.272) (3.223,-0.272) (3.254,-0.505) (3.284,-0.589) (3.314,-0.605) (3.345,-0.538) (3.375,-0.507) (3.406,-0.455) (3.436,-0.406) (3.467,-0.389) (3.497,-0.394) (3.528,-0.412) (3.558,-0.422) (3.588,-0.420) (3.619,-0.422) (3.649,-0.414) (3.680,-0.277) (3.710,-0.276) (3.741,-0.292) (3.771,-0.283) (3.802,-0.297) (3.832,-0.295) (3.862,-0.296) (3.893,-0.294) (3.923,-0.285) (3.954,-0.283) (3.984,-0.277) (4.015,-0.280) (4.045,-0.280) (4.076,-0.279) (4.106,-0.274) (4.136,-0.266) (4.167,-0.265) (4.197,-0.261) (4.228,-0.257) (4.258,-0.258) (4.289,-0.258) (4.319,-0.257) (4.350,-0.258) (4.380,-0.258) (4.411,-0.258) (4.441,-0.258) (4.471,-0.258) (4.502,-0.258) (4.532,-0.258) (4.563,-0.259) (4.593,-0.259) (4.624,-0.259) (4.654,-0.644) (4.685,-1.048) (4.715,-1.070) (4.745,-1.072) (4.776,-1.081) (4.806,-1.089) (4.837,-1.088) (4.867,-1.079) (4.898,-1.068) (4.928,-1.060) (4.959,-1.052) (4.989,-0.967) (5.019,-0.462) (5.050,-0.309) (5.080,-0.809) (5.111,-1.034) (5.141,-0.865) (5.172,-0.817) (5.202,-0.841) (5.233,-0.773) (5.263,-0.408) (5.293,-0.410) (5.324,-0.386) (5.354,-0.383) (5.385,-0.397)};
\draw[black,line width=0.35pt,dash pattern=on 1.6pt off 1.1pt] (0.620,-0.619) -- (5.400,-0.619);
\draw[black,line width=0.45pt,dash pattern=on 0.4pt off 0.9pt] (0.620,-1.044) -- (5.400,-1.044);
\draw[black,line width=0.35pt] (0.620,-1.150) rectangle (5.400,0);
\draw[black,line width=0.35pt] (0.620,-1.150) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (0.620,-1.200) {0};
\draw[black,line width=0.35pt] (1.533,-1.150) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (1.533,-1.200) {5};
\draw[black,line width=0.35pt] (2.447,-1.150) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (2.447,-1.200) {10};
\draw[black,line width=0.35pt] (3.360,-1.150) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (3.360,-1.200) {15};
\draw[black,line width=0.35pt] (4.274,-1.150) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (4.274,-1.200) {20};
\draw[black,line width=0.35pt] (5.187,-1.150) -- ++(0,-0.05);
\node[anchor=north,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (5.187,-1.200) {25\,s};
\draw[black,line width=0.35pt] (0.620,-1.150) -- ++(-0.05,0);
\node[anchor=east,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (0.570,-1.150) {0};
\draw[black,line width=0.35pt] (0.620,-0.708) -- ++(-0.05,0);
\node[anchor=east,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (0.570,-0.708) {0.5};
\draw[black,line width=0.35pt] (0.620,-0.265) -- ++(-0.05,0);
\node[anchor=east,inner sep=0.8pt,font=\fontsize{6.3}{7.4}\selectfont] at (0.570,-0.265) {1};
\node[anchor=south,rotate=90,inner sep=0pt,font=\fontsize{6.3}{7.4}\selectfont] at (0.12,-0.575) {area / p90};
\end{tikzpicture}%

